Modular Neural Network Approaches for Surgical Image Recognition

Deep learning-based applications have seen a lot of success in recent years. Text, audio, image, and video have all been explored with great success using deep learning approaches. The use of convolutional neural networks (CNN) in computer vision, in particular, has yielded reliable results. In order to achieve these results, a large amount of data is required. However, the dataset cannot always be accessible. Moreover, annotating data can be difficult and time-consuming. Self-training is a semi-supervised approach that managed to alleviate this problem and achieve state-of-the-art performances. Theoretical analysis even proved that it may result in a better generalization than a normal classifier. Another problem neural networks can face is the increasing complexity of modern problems, requiring a high computational and storage cost. One way to mitigate this issue, a strategy that has been inspired by human cognition known as modular learning, can be employed. The principle of the approach is to decompose a complex problem into simpler sub-tasks. This approach has several advantages, including faster learning, better generalization, and enables interpretability. In the first part of this paper, we introduce and evaluate different architectures of modular learning for Dorsal Capsulo-Scapholunate Septum (DCSS) instability classification. Our experiments have shown that modular learning improves performances compared to non-modular systems. Moreover, we found that weighted modular, that is to weight the output using the probabilities from the gating module, achieved an almost perfect classification. In the second part, we present our approach for data labeling and segmentation with self-training applied on shoulder arthroscopy images.

==> summary.tex <==
%\renewcommand*{\arraystretch}{1.2}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\begin{longtable}{@{\extracolsep{\fill}}>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c}
\caption{A summary of contributions presented in this survey for learning bounds in domain adaptation. \textbf{(Task)} refers to the considered learning problem; \textbf{(Framework)} specifies the statistical learning framework used in the analysis; \textbf{(Divergence)} is the metric used to compare the source and target distributions; \textbf{(Link)} stands for the dependence between the source error and the divergence term; \textbf{(Non-estim.)} indicates the presence of a non-estimable term in the bounds.} 
\endfirsthead
\endhead
\toprule
\addlinespace[.1cm]
\multirow{3}{*}{\footnotesize{\textbf{\textsc{Reference}}}}& \multicolumn{5}{c}{\footnotesize{\textbf{\textsc{Learning bounds}}}}\\
\addlinespace[.1cm]\cline{2-6}
\addlinespace[.1cm]
& \textbf{\textsc{Task}} & \textbf{\textsc{Framework}} & \textbf{\textsc{Divergence}} &	\textbf{\textsc{Link}} & \textbf{\textsc{Non-estim.}}\\
\addlinespace[.1cm]
\toprule
\addlinespace[.1cm]
\makecell{\cite{BenDavid07analysisof}\\\cite{Blitzer07Learning}\\\cite{bendavidth}} & \makecell{Binary\\ classification} & VC & $L^1$, $\hdh$ & Add. & $+$\\
\hline
\addlinespace[.1cm]
\cite{MansourMR09colt} & \makecell{Classification/\\ Regression} & Rademacher & Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\makecell{\cite{CortesMM10}\\\cite{CortesM14}\\\cite{CortesMM15}} & Regression & Rademacher & \makecell{(Generalized)\\ Discrepancy} & Add. & $+$\\
\hline
\addlinespace[.1cm]
\cite{KurokiCBHSS19} & \makecell{Classification} & Rademacher & (S-)Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MansourMR08multiple} & \makecell{Classification/\\ Regression} & -- & -- & -- & --
\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\makecell{\cite{MansourMR09}\\\cite{HoffmanMZ18}} & \makecell{Classification/\\ Regression} & -- & R\'enyi & Mult. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{DhouibR18} & \makecell{Binary classification/\\Similarity learning} & -- & $L^1$, $\chi^2$ & Mult. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoCFT19} & Binary classification & Rademacher & Discrepancy & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{ZhangZY12} & \makecell{Regression/ \\ Classification} & \makecell{Uniform \\entropy number} & IPM & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{Redko15} & Regression & Rademacher & IPM/MMD & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoHS16} & Regression & -- & IPM/Wassertein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{zhang_bridging_2019} & \makecell{Large-margin\\classification} & Rademacher & IPM & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{JohanssonSR19} & \makecell{Classification} & -- & IPM & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{ShenQZY18} & Classification & -- & Wasserstein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{CourtyFHR17} & Classification & -- & Wasserstein & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{pbda} & \makecell{Classification} & PAC-Bayes & Domain disagreement & Add. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{dalc} & \makecell{Classification} & PAC-Bayes & $\beta$-divergence & Mult. & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{li2007bayesian} & Classification & PAC-Bayes & -- & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{McNamaraB17} & \makecell{Binary classification} & VC/PAC-Bayes & -- & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MansourS14} & Classification & Robustness & $\lambda$-shift & Add. & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.05cm]
\makecell{\cite{KuzborskijO13}\\\cite{KuzborskijO17}\\\cite{simonHTL}} & Regression & Stability & -- & -- & --\\
\addlinespace[.05cm]
\hline
\addlinespace[.1cm]
\cite{PerrotH15ICML} & \makecell{Classification/\\Similarity learning} & Stability & -- & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{MorvantKAIS12} & \makecell{Classification/\\Similarity learning} & Robustness/VC & $\hdh$ & Add. & +\\
\addlinespace[.1cm]
\bottomrule
\end{longtable}
\begin{longtable}{@{\extracolsep{\fill}}>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c>{\footnotesize}c}
\caption{A summary of contributions presented in this survey for hardness results in domain adaptation. \textbf{(Type)} is the type of the obtained result; \textbf{(Setting)} points out the presence or absence of target data (either labelled or unlabelled); \textbf{(Assumptions)} indicate the considered assumptions (individual or combined); \textbf{(Proper)} specifies if the learned model is required to belong to a predefined class; \textbf{(Constr.)} indicates if the result is of a constructive nature.} 
\endfirsthead
\endhead
\toprule
\addlinespace[.1cm]
\multirow{3}{*}{\footnotesize{\textbf{\textsc{Reference}}}}& \multicolumn{5}{c}{\footnotesize{\textbf{\textsc{Hardness results}}}}\\
\addlinespace[.1cm]\cline{2-6}
\addlinespace[.1cm]
& \textbf{\textsc{Type}} & \textbf{\textsc{Setting}} & \textbf{\textsc{Assumptions}} &	\textbf{\textsc{Proper}} & \textbf{\textsc{Constr.}}\\
\addlinespace[.1cm]
\toprule
\addlinespace[.1cm]
\cite{BenDavidLLP10} & \makecell{Impossibility/\\Sample compl.} & Unlabelled target & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{BenDavidSU12} & \makecell{Impossibility/\\Sample compl.} & \makecell{No target/\\Unlabelled target} & \makecell{Cov. shift,\\$C_{\cal B}$, Lipscht.} & $+$ & $+$/--\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{BenDavidU12} & \makecell{Impossibility/\\Sample compl.} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$C_{\cal B}$, Realizab.} & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{RedkoHS19} & \makecell{Estimation/\\Sample compl.} & \makecell{Labelled target} & -- & -- & --\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{CZG19} & \makecell{Impossibility} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{JohanssonSR19} & \makecell{Impossibility} & \makecell{Unlabelled target} & \makecell{Cov. shift,\\$\hdh$, $\lambda_\Hcal$} & -- & $+$\\
\addlinespace[.1cm]
\hline
\addlinespace[.1cm]
\cite{hanneke19} & \makecell{Sample compl.} & \makecell{Labelled target} & \makecell{Relaxed cov. shift,\\Noise cond.} & -- & --\\
\bottomrule
\end{longtable}
%
